Stochastic Continuous Submodular Maximization: Boosting via Non-oblivious Function

In this paper, we revisit Stochastic Continuous Submodular Maximization in both offline and online settings, which can benefit wide applications in machine learning and operations research areas. We present a boosting framework covering gradient ascent and online gradient ascent. The fundamental ingredient of our methods is a novel non-oblivious function $F$ derived from a factor-revealing optimization problem, whose any stationary point provides a $(1-e^{-\gamma})$-approximation to the global maximum of the $\gamma$-weakly DR-submodular objective function $f\in C^{1,1}_L(\mathcal{X})$. Under the offline scenario, we propose a boosting gradient ascent method achieving $(1-e^{-\gamma}-\epsilon^{2})$-approximation after $O(1/\epsilon^2)$ iterations, which improves the $(\frac{\gamma^2}{1+\gamma^2})$ approximation ratio of the classical gradient ascent algorithm. In the online setting, for the first time we consider the adversarial delays for stochastic gradient feedback, under which we propose a boosting online gradient algorithm with the same non-oblivious function $F$. Meanwhile, we verify that this boosting online algorithm achieves a regret of $O(\sqrt{D})$ against a $(1-e^{-\gamma})$-approximation to the best feasible solution in hindsight, where $D$ is the sum of delays of gradient feedback. To the best of our knowledge, this is the first result to obtain $O(\sqrt{T})$ regret against a $(1-e^{-\gamma})$-approximation with $O(1)$ gradient inquiry at each time step, when no delay exists, i.e., $D=T$. Finally, numerical experiments demonstrate the effectiveness of our boosting methods.

==> arxiv_v3/Boosting_FW.tex <==
%Recently, the \citep{mitra2021submodular+} investigates the continuous DR-submodular maximization with concave regularization, in which they take a similar non-oblivious function to boost the approximation ratio of submodular part from $(1/2)$ to $(1-1/e)$. In this section, we demonstrate some relationships between our devised non-oblivious function $F(\boldsymbol{x})$ and that of \cite{mitra2021submodular+}. In \cite{mitra2021submodular+}, they propose an auxiliary function $G(\boldsymbol{x})$ for DR-submodular function $f(\boldsymbol{x})$, i.e., for fixed $\epsilon$, 
%\begin{equation}\label{equ:31}
 %   \begin{aligned}
  %      G(\boldsymbol{x})=\sum_{j=1}^{\epsilon^{-1}}\frac{e^{\epsilon j}f(\epsilon j*\boldsymbol{x})}{j}.
   % \end{aligned}
%\end{equation}
%We observe that $\nabla G(\boldsymbol{x})=\epsilon\sum_{j=1}^{\epsilon^{-1}}e^{\epsilon j}\nabla f(\epsilon j*\boldsymbol{x})$. Also, if assuming $\nabla f(z*\boldsymbol{x})$ is integrable w.r.t. $z\in[0,1]$, for any fixed $\boldsymbol{x}$, we have $\lim_{\epsilon\rightarrow 0}G(\boldsymbol{x})=\int_{z=0}^{1}e^{z}\nabla f(z*\boldsymbol{x})dz=e\nabla F(\boldsymbol{x})$ when $\gamma=1$. Naturally, we could view the $\nabla G(\boldsymbol{x})$ as a discrete approximation to our proposed $\nabla F(\boldsymbol{x})$. However, in \citep{mitra2021submodular+}, they do not give the motivation why they design the auxiliary function $G(\boldsymbol{x})$ in that form. In contrast, we derive the non-oblivious function $F(x)$ via the factor-revealing optimization equation~\eqref{equ:19} and from Theorem~\ref{thm:1}, we know the function $F$ satisfying $\nabla F(\boldsymbol{x})=\int_{z=0}^{1}e^{\gamma(z-1)}\nabla f(z*\boldsymbol{x})\mathrm{d}z$ is optimal in some sense. 
\blue{As discussed before}, the classical Frank-Wolfe algorithm~\citep{lacoste2016convergence}, which converges to the stationary points, achieves $(1/2)$-approximation ratio~\citep{bian2020continuous}. 
% Then, \citet{bian2017guaranteed} shift toward a variant of Frank-Wolfe algorithm with $(1-1/e)$-approximation guarantee. 
\blue{Due to the effectiveness of boosting strategy for gradient method, we also apply this} in the classical Frank-Wolfe algorithm~\citep{lacoste2016convergence} for submodular maximization. 
The precise description of our boosting Frank-Wolfe algorithm is presented in Algorithm~\ref{alg:3}.

\begin{algorithm}[t]
    \small 
	\caption{Boosting Frank-Wolfe($\delta$)}\label{alg:3}
	\hspace*{0.02in} {\bf Input:} $T$, $\gamma$, $L$, $r(\mathcal{X})$, $\rho_{t}$, $\eta_{t}$, $c>0$ and parameter $\delta$\\
    \hspace*{0.02in} {\bf Output:} $x_{l}$
	\begin{algorithmic}[1]
    	\State \textbf{Initialize:} any $\boldsymbol{x}_{1}\in\mathcal{C}$, \blue{$\boldsymbol{v}_{0}\in\mathcal{C}$}.
    	\For{$t\in [T]$}
	   % \State Sample $z_{t}$ from $\mathbf{Z}$ where $\mathrm{Pr}(\mathbf{Z}\le z)=\int_{0}^{z}\frac{\gamma e^{\gamma(u-1)}}{1-e^{-\gamma}}I(u\in[0,1])\mathrm{d}u$.
		\State \blue{Calculate $\widetilde{\nabla}F(\boldsymbol{x}_{t})$ according to \cref{alg:framework}}
		\State \blue{$\boldsymbol{v}_{t}=(1-\rho_{t})\boldsymbol{v}_{t-1}+\rho_{t}\widetilde{\nabla}F(\boldsymbol{x}_{t})$}
		\State $\boldsymbol{s}_{t+1}=\arg\max_{\boldsymbol{s}\in\mathcal{C}}\langle\boldsymbol{s},\boldsymbol{v}_{t}\rangle$
		\State $\boldsymbol{x}_{t+1}=(1-\eta_{t})\boldsymbol{x}_{t}+\eta_{t}\boldsymbol{s}_{t+1}$
	    \EndFor
	    \State Set $\triangle_{t}=\eta_{t}$ when $t<T$ and $\triangle_{T}=\frac{1+\ln(\tau)}{\eta}$ where $\tau=\max(\frac{1}{\gamma},\frac{L_{*}r^{2}(\mathcal{X})}{c})$.
    	\State Set $\triangle=\sum_{t=1}^{T}\triangle_{t}$
	    \State Choose a $l\in[T]$ with the distribution $\mathrm{Pr}(l=t)=\frac{\triangle_{t}}{\triangle}$
	\end{algorithmic}
\end{algorithm}
In Algorithm~\ref{alg:3}, besides the classical Frank-Wolfe framework, we also consider the variance reduction technique~\citep{mokhtari2018conditional} to tackle the non-vanish variance of stochastic gradient. Finally, we present the rate of convergence of Algorithm~\ref{alg:3} in Theorem~\ref{thm:8}.
\begin{theorem}[Proof in Appendix C]\label{thm:8}
Assuming that $f$ is $L$-$smooth$ and the unbiased stochastic gradient oracle $\widetilde{\nabla}f(\boldsymbol{x})$ whose variance $\mathbb{E}(\|\widetilde{\nabla}f(\boldsymbol{x})-\nabla f(\boldsymbol{x})\|^{2}|\boldsymbol{x})\le\sigma^{2}$, then, for any $\delta>0$, if we set  $\eta=O(T^{-\frac{1}{1+\delta}})$, $\rho_{t}=\frac{2}{(t+3)^{2/3(1+\delta)}}$, and $c=O(1)$ in Algorithm~\ref{alg:3}, we have
\begin{align*}
        \mathbb{E}(f(\boldsymbol{x}_{l}))\ge\bigg(1-e^{-\gamma}-O\Big(T^{-\frac{\delta}{1+\delta}}\Big)\bigg)OPT-O\big(T^{-\frac{1}{3(1+\delta)}}\big),
     \end{align*}
 where $OPT=\max_{\boldsymbol{x}\in\mathcal{C}}f(\boldsymbol{x})$.
\end{theorem}
\begin{remark}
From \cref{thm:8}, our boosting Frank-Wolfe achieves objective $(1-1/e-\epsilon^{3\delta})OPT-\epsilon$ after $O(1/\epsilon^{3(1+\delta)})$ iterations, which also efficiently improves the theoretical guarantee of the classical Frank-Wolfe algorithm~\citep{lacoste2016convergence, bian2020continuous}. 
%\blue{It is worth to mention that our boosting Frank-Wolfe method can initialize from any feasible point, different from previous methods~[???] which need to start from zero point.}
\end{remark}

